Towards Reliable Latent Knowledge Estimation in LLMs: Zero-Prompt Many-Shot Based Factual Knowledge Extraction

In this paper, we focus on the challenging task of reliably estimating factual knowledge that is embedded inside large language models (LLMs). To avoid reliability concerns with prior approaches, we propose to eliminate prompt engineering when probing LLMs for factual knowledge. Our approach, called Zero-Prompt Latent Knowledge Estimator (ZP-LKE), leverages the in-context learning ability of LLMs to communicate both the factual knowledge question as well as the expected answer format. Our knowledge estimator is both conceptually simpler (i.e., doesn't depend on meta-linguistic judgments of LLMs) and easier to apply (i.e., is not LLM-specific), and we demonstrate that it can surface more of the latent knowledge embedded in LLMs. We also investigate how different design choices affect the performance of ZP-LKE. Using the proposed estimator, we perform a large-scale evaluation of the factual knowledge of a variety of open-source LLMs, like OPT, Pythia, Llama(2), Mistral, Gemma, etc. over a large set of relations and facts from the Wikidata knowledge base. We observe differences in the factual knowledge between different model families and models of different sizes, that some relations are consistently better known than others but that models differ in the precise facts they know, and differences in the knowledge of base models and their finetuned counterparts. Code available at: https://github.com/QinyuanWu0710/ZeroPrompt_LKE

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)

SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf 

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%-tagged.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/$(PACKAGE)-tagged.cls: $(PACKAGE)-tagged.cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png


samples/sample-acmsmall-tagged.pdf:  samples/sample-acmsmall-tagged.tex   samples/$(PACKAGE)-tagged.cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls $(PACKAGE)-tagged.cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls \
	samples/$(PACKAGE)-tagged.cls \
	samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls $(PACKAGE)-tagged.cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> sections/design_old.tex <==
%\section{Making In-Context Learning work for Knowledge Estimation}
\section{Exploring the design space of IC-LKE}
\label{sec:icl_for_lke}
% \section{Designing a Maximally Minimal(\change{?the most minimalistic}) LKE}

% \begin{figure}
% \centering
% \subfloat[Correct Examples]{%
%   \includegraphics[width=0.33\textwidth]{plots/design/fake-False_incorrect-False_number.pdf}%
%   \label{fig:correct_example}%
% }
% \hfill
% \subfloat[Incorrect Examples]{%
%   \includegraphics[width=0.3\textwidth]{plots/design/fake-False_incorrect-True_number.pdf}%
%   \label{fig:incorrect_example}%
% }
% \hfill
% \subfloat[Unknown Examples]{%
%   \includegraphics[width=0.3\textwidth]{plots/design/fake-True_incorrect-False_number.pdf}%
%   \label{fig:unknown_example}%
% }
% \caption{\textbf{[How different examples in the prompt influence the accuracy]} We .}
% \label{fig:ic-lke-analysis}
% \end{figure}


% \begin{figure}
%     \centering
%     \includegraphics[width=0.35\textwidth]{plots/design/sep.pdf}
%     \caption{\textbf{[Influence of Different Separators]} 
% We replace the `[space]' token separating the subject-object pairs with semantically useful text (red highlight) and meaningless text (blue highlight). There is no such observed change over the separators across the models. %The red background depicts the effect of replacing with semantically useful text, while the blue background bars represent the impact of inserting meaningless text.
%     }
%     \label{fig:separators}
% \end{figure}

% In the previous section, we argued for LKE designs that select from a limited number of candidate prompts and that use a minimal number of additional tokens beyond those representing the subjects, relations, and objects in the standardized test. In this section, we present three concrete LKEs following these design principles.


% \color{black}
% \fi

%\textcolor{blue}{Under our learning problem framework, we can construct a relation-specific prefix \( p_r \) utilizing the training dataset \( R_{\text{train}}^r = \{ \langle x_{\text{train}}^i, r, \mathcal{Y}_{\text{train}}^i\rangle  \}_{i=1}^{n} \), to get \(\hat{y}\).}
% Subsequently, this prefix \( p_r \) is employed to ascertain \(\hat{y}(x_{\text{test}}, \mathcal{Y}_{\text{test}}, p_r)\), for all the \( \langle x_{\text{test}}, r, \mathcal{Y}_{\text{test}}\rangle  \in R_{\text{test}}^r = \{ \langle x_{\text{test}}^i, r, \mathcal{Y}_{\text{test}}^i\rangle  \}_{i}^{m} \).


% The accuracy metric for a given relation \( r \) is defined as:

% \[
% A(r) = \frac{\sum_{x, \mathcal{Y} \in R} \delta (y_c = \hat{y} (x, \mathcal{Y}, p_r))}{\lvert R \rvert}
% \]

% In this expression, \(\delta(\cdot)\) signifies the indicator function, and \( R \) represents the set of facts corresponding to the relation \( r \).



% For PB-LKE, $p_r : x, r, y$

% For IC-LKE, $p_r : \langle x_{f_1},y_{f1}...,x_{f_{50}},y_{f_{50}}\rangle $ where $x_f$ are the correct in-context samples used for evaluating $x,y$.

% For EIC-LKE, $p_r : \langle  x_{f_1},y_{f_1}...,x_{f_{10}},y_{f_{10}}\rangle ,x_1,y_1,\langle x_{f_{11}},y_{f_{11}}...,x_{f_{16}},y_{f_{16}}\rangle $ where $x_f$ are the short sequences of correct in-context samples and $x_1,y_1$ is one of the evaluation samples provided in the same context window while evaluating $x,y$.

% \color{red}
% [Bishwa] I am confused in the sentence: Subsequently, this prefix \( p_r \) is employed to certain \(\hat{y}(x_{\text{test}}, \mathcal{Y}_{\text{test}}, p_r)\), for all the \( \langle x_{\text{test}}, r, \mathcal{Y}_{\text{test}}\rangle  \in R_{\text{test}} = \{ \langle x_{\text{test}}^i, r, \mathcal{Y}_{\text{test}}^i\rangle  \}_{i}^{m} \).

% Also, since $ R = \{ \langle x^i, r, \mathcal{Y}^i\rangle  \} $ and $ y_c^i \in \mathcal{Y}^i $ is the ground-truth, the accuracy of a given relation $ r $ is 
% \begin{align*}
%     A(r) = \frac{\sum_{\langle x, r, \mathcal{Y}\rangle  \in R} \delta (y_c = \hat{y} (x, \mathcal{Y}, p_r))}{\lvert R \rvert}
% \end{align*}

% Another point, do you say $ p_r $ is a prefix \textit{for a relation $ r $}? This is for clarification only. 

% \color{black}



% {\bf A minimal \textcolor{red}{P}rompt \textcolor{red}{B}ased \textcolor{red}{LKE} (\textcolor{red}{\lkeone}):} In our first LKE design, we naturally express the tuple \( \langle x, r, \mathcal{Y} \rangle \) as a prompt. For each object $ y \in \mathcal{Y} $, we construct a prefix prompt $p_r$ = `$x$ $r$ $y$' and get the probability $ MT(x, y, p_r) $ from the LLM. The predicted object $ \hat{y} $ is the object with the maximum probability. 
% {\lkeone} is minimal with respect to a given tuple as it does not introduce any additional tokens outside the tuple. The downside of {\lkeone} is that the LLM is expected to understand the surface form representation (or semantic meaning) of the relation $ r $, which we aim to remove in our next LKE design.


% \lkeone~is minimal in the sense that it is using a fixed prompt with zero additional tokens in prompts. It also relies on a fixed function to select the correct answer using LLM responses. However, \lkeone~relies on the LLM understanding the semantics of the surface form representation of relation $r$.


% \textcolor{blue}{A simple LKE design involves generating prompts as the prefix $p_r$ corresponding to each of multiple answer choices in the multi-choices set $\mathcal{Y} = \{ y_i\}^{N}_{i=1}$, where $p_r =$ {\it ``$x$ $r$"} and obtain the predicted object $\hat{y}(x,\mathcal{Y}, p_r)$ corresponding to each subject $x$ within the context of the relation $r$.
% \textbf{Example for \lkeone:}
% \label{ex:lkeone} We provide an example of {\lkeone} on facts from a toy dataset, called \textit{Nobel dataset}, derived from Wikidata\footnote{https://www.wikidata.org/}. The dataset comprises biographical information of 954  Nobel laureates. Further details on the dataset are in Appendix \ref{appendix:nobel_dataset}. 

% For a tuple  $\langle \text{Einstein}, \text{ birth-year}, \{1879, 1880\} \rangle$, {\lkeone} constructs the following two prompts to the LLM. The correct birth year is denoted by an asterisk (*).
% \begin{align*}
%     &\text{Einstein birth-year } 1879^*\\
%     &\text{Einstein birth-year } 1880
% \end{align*}
% We obtain the predicted object (1879/1880) based on the maximum probability that the LLM puts on the two prompts.


\begin{figure}
    \centering
    \includegraphics[width=0.35\textwidth]{plots/design/fake-False_incorrect-False_number.pdf}
    \captionsetup{belowskip=-15pt,aboveskip=1pt}
    \caption{\textbf{[Influence of the number of in-context examples]} We examine how varying numbers of in-context examples influence the accuracy (calculated as defined in Eq~\ref{eq:accuracy}) across different LLMs. 
    %We randomly sample the examples from the training dataset using 5 different random seeds and calculate the average accuracy, represented by the line, and the corresponding standard deviation, shown as a shadow. 
    The vertical dashed line indicates the number of examples at which the models achieve 95\% of their respective stable accuracy at $50$ examples. %\bghosh{What is stable accuracy? Is it the accuracy when there are 50 in-context examples? Also, what is accuracy here? Is it the accuracy of the LKE? If so, we need to formally define LKE accuracy before discussing the plots}\soumi{By stable accuracy, we mean the maximum accuracy achieved after using 50 in-context examples. We can then define accuracy before the start of Section 3.1.}
    } 
    \label{fig:num-incontext}
\end{figure}

\begin{figure*}
\centering
\subfloat[(Subject, object)\\examples in a prompt]{%
  \includegraphics[width=0.2\textwidth]{plots/design/mistral-7b_unknown-False_incorrect-False_random-True.pdf}%
  \label{fig:correct_sequence}%
}
\subfloat[Distributed \\ unknown examples]{%
  \includegraphics[width=0.2\textwidth]{plots/design/mistral-7b_unknown-True_incorrect-False_random-True.pdf}%
  \label{fig:unknown_distributed}%
}
\subfloat[Continuous \\ unknown examples]{%
  \includegraphics[width=0.2 \textwidth]{plots/design/mistral-7b_unknown-True_incorrect-False_random-False.pdf}%
  \label{fig:unknown_simultaneous}%
}
\subfloat[Distributed \\ incorrect examples]{%
  \includegraphics[width=0.2\textwidth]{plots/design/mistral-7b_unknown-False_incorrect-True_random-True.pdf}%
  \label{fig:incorrect_distributed}%
}
\subfloat[Continuous \\ incorrect examples]{%
  \includegraphics[width=0.2\textwidth]{plots/design/mistral-7b_unknown-False_incorrect-True_random-False.pdf}%
  \label{fig:incorrect_simultaneous}%
}

    \captionsetup{belowskip=-15pt,aboveskip=1pt}
\caption{\textbf{[Variation in object probabilities of Nobel laureate data using Mistral-7B]} 
%We selected 200 subject-object pairs from the Nobel dataset, arranging them into a single sequence. 
Figure~\ref{fig:correct_sequence} illustrates the probability of each object at various positions in the prompt.  We show the impact on probabilities after replacing objects at distributed positions with unknown ones in Figure~\ref{fig:unknown_distributed} and incorrect ones in Figure~\ref{fig:incorrect_distributed}. We consider a continuous replacement of unknown examples in Figure~\ref{fig:unknown_simultaneous}, and incorrect examples in Figure~\ref{fig:incorrect_simultaneous}. In all plots, the horizontal dashed line shows the average probability of the correct examples (blue dots). 
%\bghosh{@Qinyuan, kindly increase the font size of these five plots in all places: ticks, labels and legends.}
%The yellow star notated the example at position 91 in the sequence.
}
\label{fig:mistral-7b-probabilities}
\end{figure*}

% We try to utilize LLMs' in-context learning ability to work for knowledge estimation, not only conveying the response format as in traditional few-shot prompting but also subtly incorporating knowledge estimation questions without explicitly stating relationships. To effectively design and utilize in-context learning for knowledge estimation(\iclke), a deeper understanding of its mechanisms is crucial. We will explore the subtleties of in-context learning, especially for latent knowledge estimation tasks, by examining the following questions:

% %will accurately respond to the known factual questions in our multiple-choice tests and struggle with the incorrect ones.
% \begin{itemize}
%     \item How many examples are required for LLMs to be able to understand a knowledge extraction task?
%     \item What are the potential consequences of including inaccurate or irrelevant examples in the prompts provided to LLMs?
%     \item What are the impacts of distributing incorrect or unknown examples intermittently versus continuously on the performance of LLMs?
%     % \item What is the effect of separators between the subject and object pairs on LKE performance?
% \end{itemize}

% We explore the factors that affect the knowledge estimation abilities of ICL-based LKEs, such as the number of in-context examples, the effect of unknown or incorrect examples, as well as the distribution of such examples within the input.
By design, IC-LKE avoids many limitations of prior works. However, IC-LKE introduces a few design choices for the input, i.e., $\prompt(\subject, \relation)$ in Equation~\eqref{eq:prompt}.
One must decide the right $n$, the number of in-context examples included in $\prompt(\subject, \relation)$. Further, it is unclear how IC-LKE would be impacted when some of the chosen examples are unknown to the model or are incorrect.
%an implicit assumption is that all $n$ in-context examples are correct. 
We study both these factors in detail by varying $n$ and introducing unknown or incorrect examples within these $n$ examples. These experiments allows us to better understand the number of in-context examples needed and how robust \iclke~is to several types of noise in these in-context examples.
We perform an in-depth empirical analysis on a \textit{Nobel Laureate} dataset for the relation \textit{`birth year'} (details in~\ref{appendix:nobel_dataset}). The dataset consists of facts formatted as $\langle \text{Person} (\subject), \text{birth-year} (\relation), \text{YYYY} (\object) \rangle$.

\if 0
\textcolor{blue}{which is divided into training and test sets; the training set is used to provide in-context examples, and the test set is used to evaluate knowledge estimation performance.}
\fi
 
%\bghosh{We mention that the representative fact has the format $\langle \text{Person}, \text{birth-year}, \text{YYYY} \rangle$ with YYYY denotes a year in four digits.}.
 % \textcolor{blue}{We separate facts into training and test set, consider the training set as in-context examples and test set to perform the knowledge extraction task}. 
 
%\textbf{Number of in-context examples.}
\textbf{More knowledgeable models need fewer in-context examples, but a small number suffices for most models.}
In Figure~\ref{fig:num-incontext}, we report knowledge estimation accuracy (Eq.~\eqref{eq:accuracy}) for different LLMs evaluated on 900 test samples, with varying numbers of in-context examples ($n$) by randomly sampling from the training set using five random seeds.
With an increasing number of in-context examples, the mean accuracy increases while the standard deviation decreases in different LLMs, i.e., the models gradually converge to a stable performance.
% Notably, some models like Mistral-7B, Llama2-7B, and Gemma-7B achieve higher estimation accuracy than others.
Using dashed vertical lines, we report the minimum number of examples required by different LLMs to achieve $95\%$ of the accuracy at $50$ in-context examples.
% of their stable accuracy, defined as the accuracy at $50$ examples.
% --- the stable accuracy of an LLM is considered as the accuracy at $50$ examples.
Interestingly, LLMs with higher estimation accuracy tend to require fewer in-context examples compared to those with lower accuracy.
A potential explanation for this behavior is that in order to infer the relation $\relation$, models need to comprehend the examples presented in the prompt. Therefore, less knowledgeable models  need to see more examples in order to infer $\relation$.
To further investigate which individual facts may be known or unknown to a model, we look at the generation probability of in-context objects in $200$ correct subject ($\subject$)-object ($\object$) pairs using the Mistral-7B model, as shown in Figure~\ref{fig:correct_sequence}. Similar results for additional models are presented in Appendix~\ref{appendix:icl}. Note that here we are only looking at probabilities of the object ($\object$) for in-context examples given previous $\subject \,\, \object$ pairs in the input to understand which of these samples are known by the LLM. 
The Mistral-7B model demonstrates a gradual increase in probability for generating correct objects as we go from left to right on the x-axis (note that for a point on the x-axis, points before it are in context, thus points on the right have more context to leverage) in Figure~\ref{fig:correct_sequence}, stabilizing at a mean probability of approximately 85\%. We also see that some objects at later positions have a lower generation probability. 
%Similar trends are observed in other models. 
%An increase in probability for the correct objects shows that in-context examples effectively convey to the LLMs that the knowledge being elicited corresponds to the relationship $\relation$ without explicitly mentioning it. 
%However, 
These low object generation probabilities suggest that the LLM may be less confident about its knowledge of the facts corresponding to them.  
%These occasional low probabilities in object generation suggest that some objects may be confidently known to the LLM. 
We can leverage the token generation probability as a signal of LLM's confidence when evaluating LKEs (see Appendix~\ref{appendix:diff_metrics}).
\if 0
\textbf{Object probability gaps emerge in sequential subject-object pairing} As illustrated in Figure \ref{fig:correct_sequence}, there is a progressive increase in object probabilities correlating with a rise in the number of in-context examples provided, suggesting that LLMs are effectively inferring the underlying relations. Additionally, the observation of consistently low probabilities for certain objects within the sequence indicates a lack of awareness of specific facts by the LLMs. This phenomenon, which we seek to quantify using LKE, highlights potential knowledge gaps of different facts in the model.
\fi

%\textbf{Injecting unknown vs.\ incorrect examples.} 
\textbf{Models are relatively robust to occasional unknown examples, but less so to occasional incorrect examples.} 
%Having established that the Mistral-7B model is familiar with over 90\% of the Nobel Laureates dataset, we investigated three aspects: (1) the generation probability for unknown facts, (2) the influence of unknown examples on the generation probability of known facts, and (3) the differential response of the LLM to in-context examples containing unknown and incorrect information. 
Next, we investigate the robustness of estimates to occasional occurrence of unknown or incorrect examples. 
To this end, we randomly chose $40$ out of the $200$ examples and replaced them first with unknown examples and next with incorrect examples. Our unknown examples are created using fictitious names and birth years~\footnote{generated via \url{https://en.namefake.com/api}}, while our incorrect examples are created by altering the birth years of known Nobel laureates. In our findings, shown in Figures~\ref{fig:unknown_distributed} and \ref{fig:incorrect_distributed}, both unknown and incorrect examples are marked by \textcolor{red}{red} dots, examples immediately following unknown/incorrect ones in \textcolor{cyan}{cyan} dots and the rest in \textcolor{blue}{blue} dots. Both the unknown and incorrect examples show generation probabilities close to zero, confirming the LLM's tendency to assign low probabilities to unknown or erroneous data. Interestingly, while unknown examples minimally impact surrounding data, incorrect examples significantly reduce the generation probability of adjacent correct examples (see one randomly marked yellow star example in Figure~\ref{fig:correct_sequence}, Figure~\ref{fig:unknown_distributed} and Figure~\ref{fig:incorrect_distributed}). This highlights a greater disruptive effect of incorrect versus unknown data on model performance. 

\if 0
To verify if LLMs demonstrate lower object probabilities for unfamiliar facts, we altered 40 examples \textcolor{red}{out of 200 examples} in our sequence by introducing incorrect and unknown data in two formats: randomly distributed and consecutive. In the incorrect scenarios, we replaced the valid object (birth year) with a false alternative.  The resulting decline in object probabilities for these incorrect and unknown inputs is prominently displayed in red in Figures \ref{fig:incorrect_distributed}, \ref{fig:incorrect_simultaneous}, \ref{fig:unknown_distributed}, and \ref{fig:unknown_simultaneous}. This approach helps elucidate the effects of error type and placement on the model’s response accuracy.
\fi
%\bghosh{Does absolute probability refer to the generation probability of the LLMs? Have we reported non-absolute probability (probability within 200 choices) anywhere in the paper? If not, we should not confuse the reader with `absolute' probability.} \soumi{It's either absolute or normalized probability. We do not usually report probability anywhere except in Section 3. We can term it as generated probability then.I changed the term above.}
%\bghosh{We need to be precise what we mean by the \textit{probability} of an example. An example consists of a pair (subject, object). Probability of an example is the generation probability of the object.}\soumi{We mention that we observe the generation probabilities of the objects above.} 

%\bghosh{In Figure 2, are we considering 200 examples as a prompt? We need to mention this.} \soumi{We do not consider 200 examples as prompt per se. It's just that we send one sequence of data which has 200 samples. These 200 samples are chosen from test set of Nobel laureate data. We observe the probabilities of each of the samples as they are processed. So, we observe the object probabilities of sample 3 given sample 1 and 2,..sample 200 given sample 1...199.}

\textbf{Models are more vulnerable to a continuous sequence of unknown or incorrect examples.} We explored the impact of different distributions of unknown and incorrect examples by setting up a more extreme scenario. In this experiment, we replaced a continuous block (rather than randomly chosen subset) of examples with unknown ones in Figure~\ref{fig:unknown_simultaneous} and incorrect ones in Figure~\ref{fig:incorrect_simultaneous}. The results indicate that the LLM is less impacted by unknown examples, quickly regaining high generation probabilities as shown in Figure~\ref{fig:unknown_simultaneous}. However, the LLM significantly struggles with a continuous block of incorrect examples, as demonstrated in Figure~\ref{fig:incorrect_simultaneous}, where such injections detrimentally affect the LLM's performance.

\textbf{Summary:} LLMs can identify the relation pattern of subject-object pairs even with a small set of in-context examples in the prompt. LLMs are relatively robust to unknown examples, but their ability to recollect factual knowledge is vulnerable to incorrect examples, particularly when they appear in a continuous sequence. 
%In addition, continuous injection of incorrect examples makes the LLM less confident about future correct examples. 
Our findings allude to the effectiveness of designing an \iclke, where we carefully place correct examples from a training dataset and proceed to estimate the latent knowledge of the LLM on examples from the test set.
Furthermore, the findings also motivate us to design a more efficient in-context learning based LKE, called {\lkethree}, that can process multiple test examples simultaneously in a single prompt where training examples are placed preceding each test example, see more details in the Appendix~\ref{appendix:design_eic_lke}.

\if 0
\bghosh{Last two paragraph will be removed.} \todo{Refine the takeaways: Based on all the previous observations, we have these takeaways: (1) LLMs can learn the patterns of subject-object pairs from some examples in the prompt, but for different LLMs, the number of examples to achieve the stable accuracy is correlated to the internal knowledge of this pattern. (2) When there are some unknown examples in the prompt, LLMs will have clear distinct generated probability on known and unknown examples, and the LLMs will be influenced to have slightly lower generated absolute probability on other examples. (3) When there are some incorrect examples in the prompt, LLMs also have clear distinct generated probability on correct and incorrect examples, but the LLMs will have a larger drop on the other examples. (4) When we replace incorrect examples, a continuous replacement will influence the following examples' generated probability significantly. (3) and (4) show that the LLMs will be confused by the incorrect examples in the prompt and will be confused more by the recent prefix.

Based on all the takeaways, we can see that the LLMs are robust to have some incorrect samples randomly distributed in the sequence, which motivates us to have a more efficient \iclke to put all the correct and incorrect choices into one sequence and get all the probability of multiple choices in one inference.
}
\fi

\if 0
\textbf{LLMs are more disrupted by incorrect facts than unknown facts}
%\bghosh{Check if the previous sentence is correct.}\soumi{Correct.}
We also observe a relative drop in probabilities of the correct samples in Figures \ref{fig:incorrect_distributed} and \ref{fig:unknown_distributed}
%that the probabilities of the correct samples relatively drop,
, especially the ones immediately `\textcolor{cyan}{following}' the incorrect or the unknown ones indicating the induced noise. One interesting thing to observe is that the effect of the noise is more for incorrect samples than that of the unknown ones.  This denotes that the LLMs get more confused by having the wrong/incorrect information about some known samples than by having some random/unknown samples. We also show a sample (marked by a yellow star) in Figures \ref{fig:correct_sequence}, \ref{fig:incorrect_distributed} and \ref{fig:unknown_distributed} whose probability drops more in case of incorrect sample injection.

\textbf{
Effect of injection patterns: continuous replacements are more disruptive than distributed.} We further observe that the correct objects' probability gets affected under different sequences of injections. Figures \ref{fig:incorrect_distributed} and \ref{fig:incorrect_simultaneous} show that having a simultaneous replacement of samples with incorrect information leads to a higher drop in probabilities of the adjacent samples compared to the distributed mode of replacement. A similar trend is observed in Figures \ref{fig:unknown_distributed} and \ref{fig:unknown_simultaneous} for the unknown samples.
\fi



%\soumi{Will write up for Q2 and Q3.}

% We assessed the impact of incorporating incorrect/unknown examples in \( p_r \) on the model's performance. Initially, it was assumed that all \( \langle x_i, y_i\rangle \) pairs in \( p_r \) correctly represented the relation \( r \). However, potential noise could introduce inaccuracies. Our results indicated a marked decrease in the accuracy of the model's responses when exposed to incorrect examples, particularly when these examples are consecutive, as illustrated in Figure~\ref{fig:factual_prob_inject} and Figure~\ref{fig:factual_prob_continuous}. In contrast, sequences of correct examples led to improved accuracy. The findings suggest two strategies: firstly, starting with about 50 factual examples can mitigate the effects of unrecognized example pairs, and secondly, interspersing short sequences of correct examples within a prompt enhances the evaluation of different answers in a single, comprehensive prompt.

% Then we come to these questions: How many examples do we need to help the model recognize the implicit patterns? What will happen if there are some incorrect or unknown factual examples in the prompt? 

% {\color{blue}TODO:


% % (a)how many examples do we need to help the model recognize the implicit relation 'birth year' -- around 10 for Llama-2-7B but 15 for Falcon-7B model

% (b)what will happen if the examples are unknown(fake)? 

% (c)what will happen if the examples are incorrect?

% Use (b) and (c) to distinct between the previous few-shot prompting: previous few-shot prompting aims to help the model understand which patterns it should generate, but if most of the examples are not correct known examples, the model can not infer the relations. Our IC-LKE communicates both the question of the relation and the format with LLMs. 

% (d)what's the influence of the in-between text? -- For Llama-2-7B, no matter which separator(both the semantic meaningful text 'birth year', 'was born in' and some random unmeaning full in-between text 'cndwijvbk' and 'ghi'.) we put in between the subject and object, the accuracy didn't change too much. For Falcon-7B, the black space in-between separator gets the highest accuracy -- we can introduce as few as possible external tokens for the model to infer the patterns.

% Then go to the final design of the IC-LKE.
% }



% We observe which prompt out of the two has a higher multi-token probability by the LLM and later compare it with ground-truth to measure accuracy.

%{\bf KG will flush this para out -- The design is maximally minimal} --  there is a fixed prompt that we are considering, it has zero additional tokens beyond the subject and objects given in the test questions themselves. Similarly, there is a fixed function we are using to process the responses from the LLMs.

%LB: premature to discuss here. Maybe move to a later section?

% {\bf Number of in-context learning examples:} 
% In order to estimate the number of in-context learning examples required for an LLM to infer the object $y$ 
% %relation $r$ between subject-object pairs,
% we conducted experiments varying the number of examples given in $p_r$ (i.e., number of $\langle x_i, y_{i,c}\rangle $) to the Llama2-7b model on the Nobel dataset \ref{appendix:nobel_dataset} .
% We focus on the relation, \emph{birth year}, to compute the probability of the predicted answers.
% Our findings are depicted in Figure~\ref{fig:factual_prob_ref}, which shows a significant increase in the probability of correct completions when the number of factual examples (on the x-axis) ranges between 5 to 10, after which the probability stabilizes.
% %In contrast, the likelihood of incorrect answers remains consistently low.
% This pattern of results is consistent across different models, including Mistral and Falcon, as shown in Appendix~\ref{appendix:icl}.
% To estimate the number of subject-object example pairs needed for an LLM's incontext learning ability to infer the implicit relationship $r$ between the pairs, we conducted an experiment using Llama2-7b \textcolor{red}{dataset ..}.
% We observe that the probabilities of completion increases sharply with the number of factual examples after 5-10 and then stabilizes.
% On the other hand, the probabilities for incorrect answers is quite low.
% We observed similar results for Mistral and Falcon. 

% {\bf Impact of incorrect and unknown examples:}
% {
% \color{blue}
% @QINYUAN would update Figure~\ref{fig:Llama2-7b-probabilities} to show the distinct of unknown and incorrect examples and 

% a. how they influence the other correct examples' probability in the sequence -- which shows that our IC-LKE is stable even though there are some unknown/incorrect examples, 

% b. how the injected examples' probability changed in the sequence, which shows that even though the test samples are distributed in the sequence, we can still distinguish the known and unknown samples. -- This finding leads us to propose the EIC-LKE
% }

% \bghosh{Is this paragraph in the right place?} \soumi{These are related to the experimental results. I'll be arranging and modifying these parts.} We assessed the impact of incorporating incorrect/unknown examples in \( p_r \) on the model's performance. Initially, it was assumed that all \( \langle x_i, y_i\rangle \) pairs in \( p_r \) correctly represented the relation \( r \). However, potential noise could introduce inaccuracies. Our results indicated a marked decrease in the accuracy of the model's responses when exposed to incorrect examples, particularly when these examples are consecutive, as illustrated in Figure~\ref{fig:factual_prob_inject} and Figure~\ref{fig:factual_prob_continuous}. In contrast, sequences of correct examples led to improved accuracy. The findings suggest two strategies: firstly, starting with about 50 factual examples can mitigate the effects of unrecognized example pairs, and secondly, interspersing short sequences of correct examples within a prompt enhances the evaluation of different answers in a single, comprehensive prompt.
% We note the probability of correct answers is also lower following an incorrect subject-object example pair. The drop in probabilities is particularly high when the incorrect examples occur in succession. However, with a succession of correct examples, the LLM begins to recognize the correct answers. Two take-aways: First, it is better to be conservative and pick a large number of initial factual examples (50) to account for cases when some of the example pairs may be unknown to the model. Second, by repeatedly having short sequences of correct examples in a long prompt, we can evaluate multiple answer choices using a single long prompt.

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.33\textwidth]{plots/design/llama2-7b_probability_distribution_ref.pdf}
%     \caption{Probabilities of completion for factual examples [Llama2-7b]}
%     \label{fig:factual_prob}
% \end{figure}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.33\textwidth]{plots/design/llama2-7b_probability_distribution_inject.pdf}
%     \caption{Probabilities of completion for factual examples with distributed incorrect alternative facts [Llama2-7b]}
%     \label{fig:factual_prob}
% \end{figure}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.33\textwidth]{plots/design/llama2-7b_probability_distribution_continues inject.pdf}
%     \caption{Probabilities of completion for factual examples with continous incorrect alternative facts [Llama2-7b]}
%     \label{fig:factual_prob}
% \end{figure}

% {\bf Talk about the more efficient in-context learning based LKE design that uses the full context window.}

% {\bf Show results that attempting to use the same context window to infer object completion probabilities for the same subject can confuse the model. So we plan to use different test subjects.}
\if 0 -- do not keep the comparison

\textbf{Comparing with traditional prompt-based estimation:} 
To benchmark our results against conventional prompt-based estimation techniques, we designed two distinct prompts for our Nobel Dataset.
These prompts encompass a few-shot prompt and a zero-shot prompt.
More details on the structure of the prompts can be found in Appendix~\ref{appendix:maunual_prompts}.
% For each prompt, we input it into the LLM to generate an answer. 
% The predicted answer for each prompt, denoted as $\hat{y}$, is the generated answer from the LLM. 
% The accuracy of each prompt, $A(r)$, is then computed based on this prediction.
For this experiment, we focus solely on the relation $r=\text{birth year}$.
% The specifics of the prompt generation parameters and their design are detailed in Appendix~\ref{appendix:maunual_prompts}.
Table~\ref{table:model-accuracy-comparison} shows the accuracy, $A(r)$, for four different models using both the manually designed tests and our LKEs.
The results indicate that our LKEs achieve comparable or higher accuracy relative to the traditional, manually designed tests.

\begin{table}[ht]
\centering
\caption{Accuracy for both traditional prompt-based as well as our latent knowledge extractors.}
\label{table:model-accuracy-comparison}
\scalebox{0.7}{
\begin{tabular}{lccccc}
\toprule
\textbf{Model} & \textbf{Few Shot} & \textbf{Zero Shot} & \textbf{\lkeone} & \textbf{\lketwo} & \textbf{\lkethree} \\
\midrule
Llama2-7b & 0.911 & 0.898 & 0.927 & 0.927 & 0.920 \\
Llama2-7b-chat & 0.687 & 0.739 & 0.647 & 0.732 & 0.697 \\
Llama2-13b & 0.950 & 0.941 & 0.897 & 0.947 & 0.948 \\
Llama2-13b-chat & 0.816 & 0.852 & 0.730 & 0.827 & 0.838 \\
\bottomrule
\end{tabular}}
\end{table}







\if 0 -- This is OLD TEXT

% \section{Key Idea: Analyze Probability of Generating Plausible But Incorrect Outputs}
\section{Designing an LKE Using Output Probability Distributions}

We consider facts as relations between entities, in analogy to much of the literature on knowledge graphs \citep{baek-etal-2023-direct, logan-etal-2019-baracks}.
Given a set of ground truth facts, we want to know which of them an LLM knows, as well as which of the facts the LLM knows are true.

% \subsection{Latent knowledge extraction}
\xhdr{Latent knowledge extraction}
Given an LLM $\model$, the goal of a \emph{latent knowledge extractor (LKE)} $\ext$ is to find facts that $\model$ has knowledge about.
We consider facts to be encoded in a knowledge graph $K = (E, F)$, consisting of \emph{entities} $E$ (such as people, places, dates) and \emph{facts} $F$, i.e. relationships between the entities.
Facts $F$ are a subset of all possible relationships $F \subseteq R = \{(e_h, a, e_t) | (e_h, e_t) \in E^2, a \in A\}$, i.e. edges between head entities $e_h$ and tail entities $e_t$, with annotations $a \in A$ from a set of relationship types $A$ (such as birth year or birth place).
Given model $\model$ and knowledge graph $K$, $\ext$ produces a set of \emph{extracted facts} $\hat{F} = \ext(\model, K), \hat{F} \subseteq R$ which $\model$ has knowledge about.
For example, $\ext$ might extract the fact (``Albert Einstein'', ``birth year'', ``1879'').

The challenge for a knowledge extractor $\ext$ is to extract facts $\hat{F}$ with high precision (high $P(f \in F | f \in \hat{F})$) and high recall (high $P(f \in \hat{F} | f \in F)$).

% \todo{Mention training and testing of $\ext$ and splitting $K$ into training, validation and test sets}


% \xhdr{Design space of a LKE}
A given LKE $\mathcal{M}_i$ takes an LLM, the head entity ($e_h$), and the relation ($a$). The LKE should then be able to extract the tail entity ($e_t$) accurately. How exactly this is achieved is left to the choice of the LKE designer. For example, one could come up with effective prompting strategies so that the LLM outputs $e_t$ conditioned on $e_h$ and $a$. Another possibility could be to make this a learning problem where using a training and a validation set (this could be, for example, different potions of the knowledge graph, $K$), one learns a classifier that can accurately predict $e_t$. The key challenge, however, is that this must work on an \textit{unseen} test set of ($e_h$, $a$, $e_t$) triplets, \ie a portion of $K$ that is unknown to the LKE designer. We intentionally do not impose any other restrictions on the design of LKEs since ultimately our goal is to see if an LLM knows certain facts.

\subsection{Our Proposal: Extracting knowledge via output probabilities}

% Language models act as next-token predictors, utilizing probability distributions over word sequences to reflect common word co-occurrences. The output, heavily dependent on the input prompt, has spurred extensive research into the careful crafting of prompts to derive desired responses. Thus, we introduced a methodology that exclusively employs forward-pass probabilities to assess Large Language Models' (LLMs) understanding of named entities and their relationships, aiming to isolate inherent knowledge from articulated outputs.

We present a simple, non-parametric LKE that 
% We propose to 
frames the problem of latent knowledge extraction as a multiple choice problem, where we determine which facts a model $\model$ knows based on the output probabilities it assigns to true facts, compared to plausible but incorrect alternative facts.

% \xhdr{Testing whether models know facts.}
% \xhdr{Computing probability distributions over plausible outputs}
A causal (autoregressive) language model $\model$ is a next-token predictor that models a probability distribution $P_{\model}(s_i | s_{[1:i-1]})$ over the $i$-th token $s_i$, given the preceding tokens $s_{[1:i-1]}$.
Each model $\model$ comes with a tokenizer $\tok$, that converts strings into sequences of tokens that can be consumed by $\model$.
To compute the probabilities of facts, we define an \emph{encoding function} $\enc(.)$ that maps fact triplets to sequences of tokens, i.e. to prompts.
Concretely, we convert fact $f = (e_h, a, e_t)$ to token sequence $s$, by tokenizing the string ``$e_h$ $a$ $e_t$'' according to $\model$'s tokenizer $\tok$, i.e. $\enc(f) = \tok(\text{``}e_h \, a \, e_t\text{''})$.
For example, for the fact $f =$ (``Albert Einstein'', ``birth year'', ``1879''), $\enc(f) = \tok($ ``Albert Einstein birth year 1879'' $)$.
We also experimented with more complex prompts, but did not observe big differences in performance, so we chose this prompting strategy, since it is the simplest possible one.
For more details, see Appendix~\ref{app:diff_prompts}.

Using $\enc(.)$, we define the probability $P_{\model}(f)$ of fact $f = (e_h, a, e_t)$ as $\frac{1}{|\enc(e_t)|} \sum_i P_{\model}(\enc(e_t)_i | \enc(e_h, a) \circ \enc(e_t)_{[1:i-1]})$, i.e. the mean probability of the tokens of $f$'s tail entity $e_t$, given the head entity $e_h$ and relationship type $a$ as prompt to $\model$.

To determine whether $\model$ knows a fact $f = (e_h, a, e_t)$, we first construct a set of alternative facts $F'_{f} = \{(e_h, a, e'_t)\} \subset R$.
We say that $\model$ knows fact $f$, if $P_{\model}(f) \rangle  P_{\model}(f')$ for all $f' \in F'_{f}$, i.e. if $\model$ assigns a higher probability to the correct tail entity $e_t$ than to all alternative entities $e'_t$, given the head entity $e_h$ and relationship type $a$.
For example, we would say that $\model$ knows Albert Einstein's birth year, if the probability of ``1879'' is higher than that of other years (e.g. ``1878'', ``1880''), given the prompt ``Albert Einstein birth year''.

We note that our proposed LKE is simple, but powerful; by fixing the prompting strategy to the simplest possible one, we can broadly apply our approach to any kind of LLM without making assumptions on how it outputs text. All we require is the computation of probabilities over a set of plausible options for $e_t$, which can be efficiently computed with a single forward pass over the LLM.

% \todo{Point out that our test is pretty simple, i.e. it needs very few fancy ingredients such as specific prompts and ways to evaluate the output}

% \vedant{shall we introduce the prompt format here? And can say on one line that we tried other prompt variations but find similar results.}

% To realize this objective, we proposed assessing the likelihood of generating plausible yet inaccurate outputs and employing the relative probability distribution to elucidate the depth of an LLM's understanding of named entities and their associations. More specifically, we constructed datasets consisting of triples: head entity, relation, tail entity. For a specific relation, such as 'birth year', we would possess a head-entity list (e.g., scientist names) and a tail-entity list (e.g., years). To discern the LLM's comprehension of a particular head entity - we take a pair of entities in [head entity, tail entity] as input to target LLM, then compute the probability of tail entity. For each head entity, we have a list of potential tail entities, the list is all the tail entities in our dataset based on one relation. For example, we have a head entity named 'Albert Einstein', a relation named 'birth year' and corresponding tail entity as '1879' and we want to test how the LLM knows the associations between head entity:'Albert Einstein' and tail entity: '1879'. The tail entity list is a unique year list contains all the scientists' birth year(in the dataset).

\textbf{Obtaining (alternative) facts.}
We propose to obtain facts from knowledge graphs, such as Wikidata \citep{10.1145/2629489}, which store entities as nodes and relationships as annotated edges between them. 
We can use such curated knowledge graphs to scalably sample a large number of factual triplets ($e_h$, $a$, $e_t$).
% We can use knowledge graphs to sample a large number of fact triplets in an automated manner.
Our multiple choice test relies on comparing the probability of correct tail entities with those of \textit{plausible but incorrect} alternatives.
In the example above, ``1878'' and ``1900'' are plausible alternatives for the correct entity ``1879'', but other entities such as ``Paris'' and ``Isaac Newton'' are not, under the relationship type $a =$ ``birth year''.
To obtain a set of plausible alternatives for fact $f$, we collect the tail entities from other facts with the same relationship type as $f$, such as the birth years of other scientists.


% \textbf{Prompt construction and output evaluation:}

% LLMs consume inputs and produce outputs as tokens.
% To test whether fact $F = (e_h, r, e_t)$ is known by a model $\gM$, we therefore need to convert $F$ into a sequence of tokens -- i.e. a prompt -- via the encoding function $\enc$ and the token probabilities produced by $\gM$ back into probabilities over tail entities.
% To keep prompts as simple as possible, we directly amalgamated $e_h$ and $r$ as the input prompt and get the probability of $e_t$ based on this prompt.


\textbf{Metrics.}
To measure the performance of our approach, evaluate it using two metrics:
\begin{itemize}
    \item \textbf{Probability Mass Function(PMF)}: We compute the probability mass of the correct fact $f$, relative to alternative facts $F'$ as $P_{\model}(f) / (P_{\model}(f) + \sum_{f' \in F'} P_{\model}(f'))$.
    The PMF quantifies model $\model$'s confidence in predicting $f$, with high PMF values indicating high confidence.
    \item \textbf{Precision}: We say that $\model$ predicts the fact $\hat{f}$ out of $\{f\} \cup F'$ to which it assigns the highest probability.
    Precision is the number of times $f$ was correctly predicted out of $\{f\} \cup F'$.
\end{itemize}

% Then we test the probability of all the years in the year list $p(y_i|x)$, where $y_i$ is the tested year, $x$ is the head entity('Albert Einstein'). Then we normalized all the tail entities' probability to get a normalized probability distribution based on the tail entity list.

% The relative probability distribution serves as an indicator of the LLM's understanding of the relationship between one entity and another. Drawing upon this indicator, we have devised four metrics designed to quantify the LLM's knowledge across various dimensions: probability mass function (PMF) and precision. The following elucidates each of these metrics:

% \begin{itemize}
%     % \item \textbf{Entropy}: Entropy measures the uncertainty associated with the predicted probability distribution. A higher entropy indicates a more uncertain prediction, implying the LLM's lack of confidence or knowlege regarding the association between two entities.
%     \item \textbf{Probability Mass Function(PMF)}: The Probability Mass Function (PMF) assesses the probability of a particular outcome occurring. Within the framework of our research, it quantifies the model's confidence in predicting the relationship interlinking two entities. A substantial probability mass allocated to a singular tail entity would denote the model’s robust conviction in that specific tail entity.
%     \item \textbf{Precision}: In our research, we choose the tail entity with the highest probability from the list as the prediction by the LLM. Precision is simply the number of correct predictions divided by the total number of entities we tested.
% \end{itemize}

% Utilizing the defined metrics, we probe the relative distribution to gain insights into the model's perception of the designated entity or context. Elevated probabilities associated with specific tokens can uncover not only the model's understanding and associations concerning the named entity but also potential biases inherent in the model. This approach offers a nuanced lens through which the intrinsic knowledge and inclinations of the LLM can be discerned.

\fi

==> sections/limitation.tex <==

\section{Limitations}

% This work, while advancing the understanding of latent factual knowledge in LLMs using an in-context learning based approach, is not without its limitations.
This study contributes to advancing our understanding of latent factual knowledge in LLMs through an innovative in-context learning approach.
However, it is essential to acknowledge the inherent limitations of our work. 
While the use of in-context learning aims to mitigate the influence of prompt engineering and the reliability issues associated with previous prompting methods, it introduces its own biases based on the selection and formulation of in-context examples. We discuss these in detail in Section~\ref{sec:icl_for_lke}. For example, the choice of which examples to include, their order, and their factual accuracy can influence model responses, and thus these in-context examples must be carefully curated for reliable latent knowledge estimation. 
\rebuttal{
Another limitation is the uncertainty regarding the application of our method to 1-N facts or N-N facts mapping. It is not clear whether our in-context learning approach can effectively handle these mappings, and we leave this line of work for future exploration.}
Our study's limitation in testing simple-format facts underlines a critical gap in assessing LLMs' complex reasoning abilities. The knowledge estimation framework employed predominantly hinges on the LLM's capacity to correctly recall or recognize factual information from a given set of triplets or structured prompts. This narrows the scope of evaluation to straightforward factual recall, thereby overlooking the models' capability to engage in more sophisticated cognitive processes such as reasoning, synthesis, and inference, which we leave as open avenues for future work. 

==> sections/sec5_why_icl.tex <==
\section{Why IC-LKE works so well in knowledge extraction?}
